Polarization Tracking in the Presence of PDL and Fast Temporal Drift

In this paper, we analyze the effectiveness of polarization tracking algorithms in optical transmission systems suffering from fast state of polarization (SOP) rotations and polarization-dependent loss (PDL). While most of the gradient descent (GD)-based algorithms in the literature may require step size adjustment when the channel condition changes, we propose tracking algorithms that can perform similarly or better without parameter tuning. Numerical simulation results show higher robustness of the proposed algorithms to SOP and PDL drift compared to GD-based algorithms, making them promising candidates to be used in aerial fiber links where the SOP can potentially drift rapidly, and therefore becomes challenging to track.

==> Figures/tikz/Fig4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{AWGN}{rgb}{0.00000,0,0}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{UDDLMS}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{SW-Kabsch}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{Louchet}{rgb}{1,0.1,0.0}%
%
% \definecolor{SW_LS}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{LS}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{LS_DDLMS}{rgb}{0.63500,0.07800,0.18400}%
% \definecolor{LS_Czegledi}{rgb}{0.30100,0.74500,0.93300}%
% \definecolor{Mcma}{rgb}{0.49400,0.18400,0.55600}%
% \definecolor{LS_SW_Kabsch}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{ML_Demod}{rgb}{0.92900,0,0.92}%
%
\newcommand\w{7}
\newcommand\h{5.5}
\newcommand\LineWidth{1.2}


\pgfplotscreateplotcyclelist{list1}{%
{color=AWGN,mark=triangle*,line width=\LineWidth pt},
{color=MCMA,mark=oplus,mark size=2.5pt,mark options=solid,line width=\LineWidth pt,densely dotted},
{color=MCMA,mark=oplus*,mark size=2.5pt,mark options=solid,line width=\LineWidth pt, densely dashed},
%{color=LS,mark=x,line width=\LineWidth pt},
{color=Louchet,mark=x,,mark size=2.5pt,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=Czegledi,mark=square,,mark options=solid,line width=\LineWidth pt,densely dotted},
{color=Czegledi,mark=square*,,mark size=2.5pt,mark options=solid,mark size=2pt,line width=\LineWidth pt,densely dashed},
{color=SW-Kabsch,mark=triangle,mark size=2.5pt,mark options=solid,line width=\LineWidth pt,densely dashed}
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
font=\small,
xmode=log,
xmin=1e-08,
xmax=0.001,
xminorticks=true,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\Deltaptot\cdot T$},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER  $\eta$ = 18 dB},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black},
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black}
]
\pgfplotsset{cycle list name=list1}

\addplot %[color=AWGN, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00116139984130859\\
1e-07	0.00116114044189453\\
3.57142857142857e-07	0.00116139221191406\\
1e-06	0.00116106414794922\\
3.57142857142857e-06	0.00116110992431641\\
1e-05	0.00116070556640625\\
3.57142857142857e-05	0.0011612548828125\\
6.07142857142857e-05	0.00116164398193359\\
0.0001	0.00116092681884766\\
0.000178571428571429	0.00116120910644531\\
0.000357142857142857	0.00116099548339844\\
0.001	0.00116210174560547\\
};
\addlegendentry{AWGN ($\Hb$ is known)}

\addplot %[color=MCMA, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00165279048490393\\
1e-07	0.00180721930253835\\
3.57142857142857e-07	0.00233057086320986\\
1e-06	0.00416183323049427\\
3.57142857142857e-06	0.0214221472797293\\
1e-05	0.122039069980212\\
3.57142857142857e-05	0.69367265260963\\
6.07142857142857e-05	0.792566762058767\\
0.0001	0.830544947764846\\
0.000178571428571429	0.849878151662801\\
0.000357142857142857	0.860237276325028\\
0.001	0.867360443839231\\
};
\addlegendentry{MCMA $\smash{\mu= 10^{-3}}$}

\addplot %[color=MCMA, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00141986461478523\\
1e-07	0.00181232752183371\\
3.57142857142857e-07	0.00232188889971105\\
1e-06	0.00344746112139216\\
3.57142857142857e-06	0.00727839193532677\\
1e-05	0.0225552822960294\\
3.57142857142857e-05	0.0606591669101652\\
6.07142857142857e-05	0.108133964806337\\
0.0001	0.227371960325963\\
0.000178571428571429	0.482493360605175\\
0.000357142857142857	0.706620799649362\\
0.001	0.822459920132463\\
};
\addlegendentry{MCMA opt. $\mu$}

% \addplot %[color=UDDLMS, line width=2.0pt]
%   table[row sep=crcr]{%
% 1e-08	0.00124018700691536\\
% 1e-07	0.00125943962858349\\
% 3.57142857142857e-07	0.00131039576637122\\
% 1e-06	0.00143156878023441\\
% 3.57142857142857e-06	0.00189876140385052\\
% 1e-05	0.00241665855004708\\
% 3.57142857142857e-05	0.0036831596376741\\
% 6.07142857142857e-05	0.00425004869971754\\
% 0.0001	0.0187834567059511\\
% 0.000178571428571429	0.184101774293042\\
% 0.000357142857142857	0.468560663614818\\
% 0.001	0.714877812408688\\
% };
% \addlegendentry{UDDLMS}
\addplot %[color=Louchet, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00162006915359891\\
1e-07	0.00162741469432811\\
3.57142857142857e-07	0.00164837180611019\\
1e-06	0.00177679296126749\\
3.57142857142857e-06	0.00230447063407032\\
1e-05	0.00428927632219733\\
3.57142857142857e-05	0.0248860832440505\\
6.07142857142857e-05	0.149208069543197\\
0.0001	0.553496461153859\\
0.000178571428571429	0.763931812278822\\
0.000357142857142857	0.83112380279861\\
0.001	0.855146293951495\\
};
\addlegendentry{\ac{DD-Kabsch}}

\addplot %[color=Czegledi, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00118476456945892\\
1e-07	0.00122301538330603\\
3.57142857142857e-07	0.00133168790825337\\
1e-06	0.0016525989914679\\
3.57142857142857e-06	0.00362984850741505\\
1e-05	0.0185478786782698\\
3.57142857142857e-05	0.703349603183047\\
6.07142857142857e-05	0.800029596374391\\
0.0001	0.829745058405498\\
0.000178571428571429	0.844806256516096\\
0.000357142857142857	0.852598374433498\\
0.001	0.858890811506628\\
};
\addlegendentry{\ac{DD-Czegledi} $\smash{\mu=10^{-3}}$}

\addplot %[color=Czegledi, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00118537547482225\\
1e-07	0.00122474107983507\\
3.57142857142857e-07	0.00129628908152333\\
1e-06	0.00141086328365962\\
3.57142857142857e-06	0.00171039901301906\\
1e-05	0.002240649654232\\
3.57142857142857e-05	0.00498658322781728\\
6.07142857142857e-05	0.0109313009317879\\
0.0001	0.0445932112593747\\
0.000178571428571429	0.268354071296386\\
0.000357142857142857	0.527018725041395\\
0.001	0.771657503003149\\
};
\addlegendentry{\ac{DD-Czegledi} opt. $\mu$}

\addplot %[color=SW-Kabsch, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00135058114996266\\
1e-07	0.00135571085354372\\
3.57142857142857e-07	0.00136138437063732\\
1e-06	0.00138498750040583\\
3.57142857142857e-06	0.00147836920879192\\
1e-05	0.00172030940553878\\
3.57142857142857e-05	0.0030423038213045\\
6.07142857142857e-05	0.00600539755202753\\
0.0001	0.0433418720171423\\
0.000178571428571429	0.407241250284082\\
0.000357142857142857	0.682731348008181\\
0.001	0.818800688289341\\
};
\addlegendentry{SW-Kabsch}



\end{axis}
\end{tikzpicture}%

==> Figures/tikz/Fig5.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{SW_LS}{rgb}{0.92900,0,0.92}%
\definecolor{LS}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{LS_DDLMS}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{LS_Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{LS_SW_Kabsch}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{ML_Demod}{rgb}{0.85000,0.32500,0.09800}%



%
\newcommand\w{5}
\newcommand\h{4.5}
\newcommand\LineWidth{1}


\pgfplotscreateplotcyclelist{list1}{%
{color=ML_Demod,mark=triangle*,line width=\LineWidth pt},
{color=MCMA,mark=+,line width=\LineWidth pt},
{color=LS,mark=x,line width=\LineWidth pt},
{color=LS_DDLMS,mark=star,line width=\LineWidth pt},
{color=LS_Czegledi,mark=o,line width=\LineWidth pt},
{color=LS_SW_Kabsch,mark=square,line width=\LineWidth pt},
{color=SW_LS,mark=diamond,line width=\LineWidth pt},
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
font=\small,
xmode=log,
xmin=1e-08,
xmax=0.001,
xtick={1e-08,1e-07,1e-06,1e-05,0.0001,0.001},
xticklabels={{$\text{10}^{\text{-8}}$},{$\text{10}^{\text{-7}}$},{$\text{10}^{\text{-6}}$},{$\text{10}^{\text{-5}}$},{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$}},
xminorticks=true,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\Deltaptot\cdot T  $},
ymode=log,
ymin=1e-03,
ymax=1,
ytick={0.0001,0.001,0.01,0.1,1},
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black},
legend style={at={(0.2,1.1)}, font=\footnotesize,anchor=south west, legend cell align=left, align=left, draw=white!15!black},
legend columns=7
]
\pgfplotsset{cycle list name=list1}

\addplot%[ line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.0010\\
1e-07	0.0010\\
3.57142857142857e-07	0.0010\\
1e-06	0.0010\\
3.57142857142857e-06	0.0010\\
1e-05	0.0010\\
3.57142857142857e-05	0.0010\\
6.07142857142857e-05	0.0010\\
0.0001	0.0010\\
0.000178571428571429	0.0010\\
0.000357142857142857	0.0010\\
0.001	0.0010\\
};
\addlegendentry{ML ($\Hb$ is known)}

\addplot %[color=MCMA, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00207855952354497\\
1e-07	0.00286861930265117\\
3.57142857142857e-07	0.00366158136847485\\
1e-06	0.00505100113335852\\
3.57142857142857e-06	0.00978955087890842\\
1e-05	0.0281847929953999\\
3.57142857142857e-05	0.0680271783817418\\
6.07142857142857e-05	0.116244249872219\\
0.0001	0.511814595879908\\
0.000178571428571429	0.604489321984933\\
0.000357142857142857	0.717262272494944\\
0.001	0.825143336518589\\
};
\addlegendentry{MCMA}

\addplot %[line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00190715\\
1e-07	0.002485\\
3.57142857142857e-07	0.00500895\\
1e-06	0.0163934\\
3.57142857142857e-06	0.09060795\\
1e-05	0.2470074\\
3.57142857142857e-05	0.51200455\\
6.07142857142857e-05	0.61301145\\
0.0001	0.6984913\\
0.000178571428571429	0.7774962\\
0.000357142857142857	0.84285285\\
0.001	0.8932456\\
};
\addlegendentry{LS}

\addplot %[color=LS_DDLMS, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.0011419\\
1e-07	0.0012323\\
3.57142857142857e-07	0.0015566\\
1e-06	0.00171175\\
3.57142857142857e-06	0.00208725\\
1e-05	0.00356035\\
3.57142857142857e-05	0.018226\\
6.07142857142857e-05	0.1351747\\
0.0001	0.33500135\\
0.000178571428571429	0.6898658\\
0.000357142857142857	0.83627945\\
0.001	0.89798245\\
};
\addlegendentry{LS-DDLMS}

\addplot %[color=LS_Czegledi, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00146165\\
1e-07	0.00149405\\
3.57142857142857e-07	0.00156355\\
1e-06	0.00169765\\
3.57142857142857e-06	0.002108\\
1e-05	0.00286885\\
3.57142857142857e-05	0.0069005\\
6.07142857142857e-05	0.01253645\\
0.0001	0.028918\\
0.000178571428571429	0.1131839\\
0.000357142857142857	0.5535862\\
0.001	0.8641479\\
};
\addlegendentry{\ac{LS}-\ac{DD-Czegledi}}

\addplot %[color=LS_SW_Kabsch, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00164725\\
1e-07	0.00164695\\
3.57142857142857e-07	0.00164865\\
1e-06	0.00169535\\
3.57142857142857e-06	0.0018757\\
1e-05	0.00234135\\
3.57142857142857e-05	0.0046626\\
6.07142857142857e-05	0.0080678\\
0.0001	0.02190435\\
0.000178571428571429	0.1722615\\
0.000357142857142857	0.6628325\\
0.001	0.87474155\\
};
\addlegendentry{LS-SW-Kabsch}

\addplot %[color=SW_LS, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00135685\\
1e-07	0.00135405\\
3.57142857142857e-07	0.0013662\\
1e-06	0.00139565\\
3.57142857142857e-06	0.0015097\\
1e-05	0.00177815\\
3.57142857142857e-05	0.0032408\\
6.07142857142857e-05	0.00767605\\
0.0001	0.03903035\\
0.000178571428571429	0.3028537\\
0.000357142857142857	0.74237825\\
0.001	0.88325345\\
};
\addlegendentry{SW-LS}

\end{axis}
%=================================================================
%                   Figure 2
%=================================================================
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(\w cm+1cm,0cm)},
font=\small,
scale only axis,
xmode=log,
xmin=1e-08,
xmax=0.001,
xtick={1e-08,1e-07,1e-06,1e-05,0.0001,0.001},
xticklabels={{$\text{10}^{\text{-8}}$},{$\text{10}^{\text{-7}}$},{$\text{10}^{\text{-6}}$},{$\text{10}^{\text{-5}}$},{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$}},
xminorticks=true,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\Deltaptot\cdot T $},
ymode=log,
ymin=1e-03,
ymax=1,
ytick={0.0001,0.001,0.01,0.1,1},
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
yminorticks=true,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black}
]
\pgfplotsset{cycle list name=list1}
\addplot%[ line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.0010\\
1e-07	0.0010\\
3.57142857142857e-07	0.0010\\
1e-06	0.0010\\
3.57142857142857e-06	0.0010\\
1e-05	0.0010\\
3.57142857142857e-05	0.0010\\
6.07142857142857e-05	0.0010\\
0.0001	0.0010\\
0.000178571428571429	0.0010\\
0.000357142857142857	0.0010\\
0.001	0.0010\\
};
%\addlegendentry{ML (H is known)}

\addplot %[color=MCMA, line width=1.0pt]
  table[row sep=crcr]{%
1e-08	0.00302559612435832\\
1e-07	0.00432559612435832\\
3.57142857142857e-07	0.00553867863730305\\
1e-06	0.00715949243316518\\
3.57142857142857e-06	0.0133135180781795\\
1e-05	0.0345912131380697\\
3.57142857142857e-05	0.079279817329274\\
6.07142857142857e-05	0.134260983577413\\
0.0001	0.567633002955621\\
0.000178571428571429	0.644526600591124\\
0.000357142857142857	0.739611602480055\\
0.001	0.82917909286873\\
};
%\addlegendentry{MCMA}

\addplot %[color=LS, line width=1.0pt]
  table[row sep=crcr]{%
1e-08	0.0028831\\
1e-07	0.00352025\\
3.57142857142857e-07	0.0066002\\
1e-06	0.01971585\\
3.57142857142857e-06	0.09840505\\
1e-05	0.257999\\
3.57142857142857e-05	0.52010825\\
6.07142857142857e-05	0.61995585\\
0.0001	0.70397815\\
0.000178571428571429	0.78113645\\
0.000357142857142857	0.8448809\\
0.001	0.89430725\\
};
%\addlegendentry{LS}

\addplot %[color=LS_DDLMS, line width=1.0pt]
  table[row sep=crcr]{%
1e-08	0.0018645\\
1e-07	0.00192205\\
3.57142857142857e-07	0.0023925\\
1e-06	0.00259065\\
3.57142857142857e-06	0.00328985\\
1e-05	0.005415\\
3.57142857142857e-05	0.03449575\\
6.07142857142857e-05	0.1851322\\
0.0001	0.39023875\\
0.000178571428571429	0.7020143\\
0.000357142857142857	0.84000255\\
0.001	0.8992777\\
};
%\addlegendentry{LS-DDLMS}

\addplot %[color=LS_Czegledi, line width=1.0pt]
  table[row sep=crcr]{%
1e-08	0.0022712\\
1e-07	0.00226245\\
3.57142857142857e-07	0.0024051\\
1e-06	0.0027108\\
3.57142857142857e-06	0.00431015\\
1e-05	0.0096166\\
3.57142857142857e-05	0.0421965\\
6.07142857142857e-05	0.09055595\\
0.0001	0.1648378\\
0.000178571428571429	0.33236645\\
0.000357142857142857	0.70213885\\
0.001	0.8731904\\
};
%\addlegendentry{LS-Czegledi}



\addplot %[color=LS_SW_Kabsch, line width=1.0pt]
  table[row sep=crcr]{%
1e-08	0.0024845\\
1e-07	0.00243\\
3.57142857142857e-07	0.0025071\\
1e-06	0.00269405\\
3.57142857142857e-06	0.00394055\\
1e-05	0.00836425\\
3.57142857142857e-05	0.03609975\\
6.07142857142857e-05	0.06311085\\
0.0001	0.1228633\\
0.000178571428571429	0.32313605\\
0.000357142857142857	0.7069003\\
0.001	0.8788283\\
};
%\addlegendentry{LS-SW-Kabsch}

\addplot %[color=SW_LS, line width=1.0pt]
  table[row sep=crcr]{%
1e-08	0.0021701\\
1e-07	0.00208685\\
3.57142857142857e-07	0.00211595\\
1e-06	0.0021506\\
3.57142857142857e-06	0.00244265\\
1e-05	0.00281195\\
3.57142857142857e-05	0.00505075\\
6.07142857142857e-05	0.01164135\\
0.0001	0.05507435\\
0.000178571428571429	0.3339967\\
0.000357142857142857	0.75108315\\
0.001	0.8838229\\
};
%\addlegendentry{SW-LS}
\end{axis}
%=================================================================
%                   Figure 3
%=================================================================
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(2*\w cm+2cm,0cm)},
font=\small,
scale only axis,
xmode=log,
xmin=1e-08,
xmax=1e-3,
xtick={1e-08,1e-07,1e-06,1e-05,0.0001,0.001},
xticklabels={{$\text{10}^{\text{-8}}$},{$\text{10}^{\text{-7}}$},{$\text{10}^{\text{-6}}$},{$\text{10}^{\text{-5}}$},{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$}},
xminorticks=true,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\Deltaptot\cdot T $},
ymode=log,
ymin=1e-03,
ymax=1,
ytick={0.0001,0.001,0.01,0.1,1},
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
yminorticks=true,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black},
]
\pgfplotsset{cycle list name=list1}
\addplot %[color=ML_Demod, line width=\LineWidth pt, mark=*]
  table[row sep=crcr]{%
1e-08	0.0010\\
1e-07	0.0010\\
3.57142857142857e-07	0.0010\\
1e-06	0.0010\\
3.57142857142857e-06	0.0010\\
1e-05	0.0010\\
3.57142857142857e-05	0.0010\\
6.07142857142857e-05	0.0010\\
0.0001	0.0010\\
0.000178571428571429	0.0010\\
0.000357142857142857	0.0010\\
0.001	0.0010\\
};

\addplot %[color=MCMA, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00400171114913665\\
1e-07	0.00500171114913665\\
3.57142857142857e-07	0.00700171114913665\\
1e-06	0.00856980155114558\\
3.57142857142857e-06	0.0164790884241872\\
1e-05	0.0442506500144448\\
3.57142857142857e-05	0.102764172537168\\
6.07142857142857e-05	0.199075590568679\\
0.0001	0.612248327740616\\
0.000178571428571429	0.675796295473233\\
0.000357142857142857	0.758421020467122\\
0.001	0.834436154136759\\
};

\addplot %[color=LS, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.0034808\\
1e-07	0.00422515\\
3.57142857142857e-07	0.00798875\\
1e-06	0.0227568\\
3.57142857142857e-06	0.1084674\\
1e-05	0.2718634\\
3.57142857142857e-05	0.5329413\\
6.07142857142857e-05	0.62987975\\
0.0001	0.71196865\\
0.000178571428571429	0.78728705\\
0.000357142857142857	0.84888925\\
0.001	0.8965276\\
};

\addplot %[color=LS_DDLMS, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.0023613\\
1e-07	0.00241315\\
3.57142857142857e-07	0.00303945\\
1e-06	0.00324005\\
3.57142857142857e-06	0.0045501\\
1e-05	0.0083949\\
3.57142857142857e-05	0.0685825\\
6.07142857142857e-05	0.24222665\\
0.0001	0.4469405\\
0.000178571428571429	0.71783245\\
0.000357142857142857	0.8448398\\
0.001	0.9012879\\
};

\addplot %[color=LS_Czegledi, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00278135\\
1e-07	0.0027673\\
3.57142857142857e-07	0.00305975\\
1e-06	0.00371195\\
3.57142857142857e-06	0.0091905\\
1e-05	0.02889655\\
3.57142857142857e-05	0.1087911\\
6.07142857142857e-05	0.20204505\\
0.0001	0.31489845\\
0.000178571428571429	0.49502545\\
0.000357142857142857	0.7677778\\
0.001	0.8823278\\
};



\addplot %[color=LS_SW_Kabsch, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.00298635\\
1e-07	0.0029206\\
3.57142857142857e-07	0.00314235\\
1e-06	0.00368995\\
3.57142857142857e-06	0.0087253\\
1e-05	0.0268123\\
3.57142857142857e-05	0.10027825\\
6.07142857142857e-05	0.1545716\\
0.0001	0.25198955\\
0.000178571428571429	0.45527175\\
0.000357142857142857	0.74802855\\
0.001	0.8830545\\
};

\addplot %[color=SW_LS, line width=\LineWidth pt]
  table[row sep=crcr]{%
1e-08	0.0027395\\
1e-07	0.00260275\\
3.57142857142857e-07	0.00264225\\
1e-06	0.00260675\\
3.57142857142857e-06	0.0032572\\
1e-05	0.00373715\\
3.57142857142857e-05	0.00774865\\
6.07142857142857e-05	0.01949065\\
0.0001	0.0801805\\
0.000178571428571429	0.37396155\\
0.000357142857142857	0.7632038\\
0.001	0.8860483\\
};
\end{axis}

\begin{axis}[%
width=5.5cm,
height=4cm,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\node at (0.5*\w,1*\h){{(a)}};
\node at (\w+1+0.5*\w,1*\h){{(b)}};
\node at (2*\w+2+0.5*\w,1*\h){{(c)}};

\node at (0.25*\w,.85*\h)[font=\small]{$\bar{\rho}={1.0}$ {dB}};
a\node at (0.25*\w,.75*\h)[font=\small]{{SNR}$={17.75}$ {dB}};
%\draw [black,very thick](0.02*\w,0.92*\h) rectangle (0.5*\w,.78*\h);

\node at (\w+1+0.25*\w,.85*\h)[font=\small]{$\bar{\rho}={3.0}$ {dB}};
\node at (\w+1+0.25*\w,.75*\h)[font=\small]{{SNR}$={18}$ {dB}};
%\draw [black,very thick](\w+1+0.02*\w,0.92*\h) rectangle  (\w+1+0.5*\w,.78*\h);

\node at (2*\w+2+0.25*\w,.85*\h)[font=\small]{$\bar{\rho}={5.0}$ {dB}};
\node at (2*\w+2+0.25*\w,.75*\h)[font=\small]{{SNR}$={18.75}$ {dB}};
%\draw [black,very thick](2*\w+2+0.02*\w,0.92*\h) rectangle (2*\w+2+0.5*\w,.78*\h);
\end{tikzpicture}%

==> Figures/tikz/Fig6.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{AWGN}{rgb}{0.00000,0,0}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{UDDLMS}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{SW-Kabsch}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{Louchet}{rgb}{0.30100,0.74500,0.93300}%
%
% \definecolor{SW_LS}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{LS}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{LS_DDLMS}{rgb}{0.63500,0.07800,0.18400}%
% \definecolor{LS_Czegledi}{rgb}{0.30100,0.74500,0.93300}%
% \definecolor{Mcma}{rgb}{0.49400,0.18400,0.55600}%
% \definecolor{LS_SW_Kabsch}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{ML_Demod}{rgb}{0.92900,0,0.92}%
%
\newcommand\w{5}
\newcommand\h{4.5}
\newcommand\LineWidth{1.5}

\newcommand\xMax{20}
\newcommand\xMin{14}
\newcommand\yMax{1}

\pgfplotscreateplotcyclelist{list1}{%
{color=AWGN,mark=triangle*,mark options=solid,line width=\LineWidth pt},
{color=MCMA,mark=+,mark options=solid,line width=\LineWidth pt,densely dashed},
%{color=LS,mark=x,line width=\LineWidth pt},
{color=Louchet,mark=square,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=Czegledi,mark=star,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=SW-Kabsch,mark=o,mark options=solid,line width=\LineWidth pt,densely dashed}
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0*\w cm,0*\w cm)},
scale only axis,
font=\small,
xmin=\xMin,
xmax=\xMax,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
%tick label style={font =\thin},
xticklabels={$\text{13}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black},
legend style={at={(0.53,1.1)},font=\footnotesize, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
legend columns=5
]

\pgfplotsset{cycle list name=list1}
%+++++++++++ AWGN+++++++++++ 
\addplot %[color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
12	0.20400341796875\\
13	0.129314956665039\\
14	0.0726002578735352\\
15	0.0351884613037109\\
16	0.014272819519043\\
17	0.00464485931396484\\
18	0.00116139984130859\\
19	0.000215545654296875\\
20	3.65753173828125e-05\\
21	1.60369873046875e-05\\
22	1.45111083984375e-05\\
};
\addlegendentry{AWGN ($\Hb$ is known)}

%+++++++++++ MCMA +++++++++++ 
\addplot %[color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
12	0.226635271582091\\
13	0.14468264017402\\
14	0.0823198759780527\\
15	0.0403916187786111\\
16	0.0166090305509561\\
17	0.00553118405246583\\
18	0.00141986461478523\\
19	0.000264155384565437\\
20	4.77257231908056e-05\\
21	2.27265348527645e-06\\
22	4.44790753546963e-05\\
};
\addlegendentry{MCMA}

%+++++++++++ UDDLMS +++++++++++ 
% \addplot %[color=mycolor3, line width=2.0pt]
%   table[row sep=crcr]{%
% 12	0.207613640790883\\
% 13	0.132046078049414\\
% 14	0.0745016395571572\\
% 15	0.0363553780721405\\
% 16	0.0148592253498263\\
% 17	0.00491150449660725\\
% 18	0.00124018700691536\\
% 19	0.000225463458978605\\
% 20	2.71257426706925e-05\\
% 21	1.67202363559625e-06\\
% 22	8.11661959027304e-08\\
% };
% \addlegendentry{UDDLMS}

%+++++++++++ Louchet +++++++++++ 
\addplot %[color=mycolor6, line width=2.0pt]
  table[row sep=crcr]{%
12	0.224926796207915\\
13	0.145109379565598\\
14	0.0834432729456836\\
15	0.0417307717281906\\
16	0.0175860767507549\\
17	0.00602338398103958\\
18	0.00162006915359891\\
19	0.000492102529138665\\
20	0.000164353430083439\\
21	4.15083925846563e-05\\
22	1.15083925846563e-05\\
};
\addlegendentry{\ac{DD-Kabsch}}

%+++++++++++ Czegledi +++++++++++ 
\addplot %[color=mycolor4, line width=2.0pt]
  table[row sep=crcr]{%
12	0.206683622284991\\
13	0.131233661244765\\
14	0.0738241290867179\\
15	0.0358561735008604\\
16	0.0151569835394955\\
17	0.0047626862764196\\
18	0.00118537547482225\\
19	0.000211072692445051\\
20	2.41063601831109e-05\\
21	1.47722476542969e-06\\
22	1.13632674263823e-07\\
};
\addlegendentry{\ac{DD-Czegledi}}

%+++++++++++ SW-Kabsch +++++++++++ 
\addplot %[color=mycolor5, line width=2.0pt]
  table[row sep=crcr]{%
12	0.225414166747833\\
13	0.142929620791533\\
14	0.0804707314697575\\
15	0.0392832537904613\\
16	0.0160782929125678\\
17	0.00532446186812116\\
18	0.00135058114996266\\
19	0.000246842634979384\\
20	2.99016265705659e-05\\
21	1.80188954904061e-06\\
22	9.73994350832765e-08\\
};
\addlegendentry{SW-Kabsch}


\end{axis}
%=================================================================
%                   Figure 2 Deltap_T = 1 e-6
%=================================================================
% \begin{axis}[%
% width=\w cm,
% height=\h cm,
% at={(6cm,0cm)},
% scale only axis,
% xmin = \xMin=12,
% xmax=\xMax,
% xlabel style={font=\color{white!15!black}},
% xlabel={$\text{SNR}$ (dB)},
% ymode=log,
% ymin=0.001,
% ymax = \yMax=1,
% yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
% xticklabels={$\text{13}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
% yminorticks=true,
% ylabel style={font=\color{white!15!black}},
% %ylabel={SER},
% axis background/.style={fill=white},
% title style={font=\bfseries},
% %title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
% xmajorgrids,
% ymajorgrids,
% yminorgrids,
% axis background/.style={fill=white},
% axis x line*=bottom,
% axis y line*=left,
% grid style={dotted,white!70!black}
% ]
% \pgfplotsset{cycle list name=list1}
% %+++++++++++ AWGN+++++++++++ 
% \addplot %[color=ML_Demod, line width=1.0pt, mark=*]
%   table[row sep=crcr]{%
% 12	0.203995956420898\\
% 13	0.129312828063965\\
% 14	0.0725890197753906\\
% 15	0.0351843795776367\\
% 16	0.0142663269042969\\
% 17	0.00464344024658203\\
% 18	0.00116106414794922\\
% 19	0.000215476989746094\\
% 20	3.66592407226562e-05\\
% 21	1.6082763671875e-05\\
% 22	1.4495849609375e-05\\
% };

% %+++++++++++  MCMA+++++++++++ 
% \addplot %[color=Mcma, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.251058358494854\\
% 13	0.167486875426123\\
% 14	0.100821588584786\\
% 15	0.0539323479757151\\
% 16	0.0251784357650726\\
% 17	0.010106952696341\\
% 18	0.00344746112139216\\
% 19	0.000986153046978995\\
% 20	0.000241014902113568\\
% 21	5.13863186260186e-05\\
% 22	1.03324567384176e-05\\
% };
% %\addlegendentry{MCMA}
% %+++++++++++  UDDLMS+++++++++++ 
% % \addplot %[color=LS, line width=1.0pt]
% %   table[row sep=crcr]{%
% % 12	0.216066182916139\\
% % 13	0.138072960293497\\
% % 14	0.0783778448751664\\
% % 15	0.0385969449043862\\
% % 16	0.0159969319177949\\
% % 17	0.00538445180351287\\
% % 18	0.00141086328365962\\
% % 19	0.00027109509431512\\
% % 20	3.57780591539236e-05\\
% % 21	2.8895165741372e-06\\
% % 22	1.29865913444369e-07\\
% % };
% % %\addlegendentry{UDDLMS}
% %+++++++++++  Louchet+++++++++++ 
% \addplot %[color=LS_DDLMS, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.227444108957502\\
% 13	0.147282774909906\\
% 14	0.0851328771793124\\
% 15	0.042989837992273\\
% 16	0.0183534950163956\\
% 17	0.00642382552514529\\
% 18	0.00177679296126749\\
% 19	0.000421845069965261\\
% 20	0.000164353430083439\\
% 21	4.15083925846563e-05\\
% 22	1.15083925846563e-05\\
% };

%% +++++++++++ Czegledi+++++++++++ 
% \addplot %[color=LS_Czegledi, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.226052157397487\\
% 13	0.143448418882504\\
% 14	0.080885815395604\\
% 15	0.0395526443946625\\
% 16	0.016229951949612\\
% 17	0.00540018181227882\\
% 18	0.00138498750040583\\
% 19	0.000257085808902309\\
% 20	3.28073763838836e-05\\
% 21	2.32135320281809e-06\\
% 22	1.29865913444369e-07\\
% };
%% +++++++++++ SW-Kabsch+++++++++++ 

% \addplot %[color=LS_SW_Kabsch, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.227444108957502\\
% 13	0.147282774909906\\
% 14	0.0851328771793124\\
% 15	0.042989837992273\\
% 16	0.0183534950163956\\
% 17	0.00642382552514529\\
% 18	0.00177679296126749\\
% 19	0.000421845069965261\\
% 20	0.000164353430083439\\
% 21	4.15083925846563e-05\\
% 22	1.15083925846563e-05\\
% };
% %\addlegendentry{SW-Kabsch}

% \end{axis}
%=================================================================
%                   Figure 2 Deltap_T = 3.57 e-6
%=================================================================
%-************
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(\w cm+1cm,0cm)},
scale only axis,
font=\small,
xmin =\xMin,
xmax=\xMax,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax=1,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
xticklabels={$\text{13}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
%ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black}
]
%+++++++ AWGN +++++++++
\pgfplotsset{cycle list name=list1}
\addplot %AWGN
  table[row sep=crcr]{%
12	0.203999794006348\\
13	0.129312927246094\\
14	0.0725995941162109\\
15	0.0351876449584961\\
16	0.0142747344970703\\
17	0.00464553070068359\\
18	0.0011612548828125\\
19	0.000215400695800781\\
20	3.66744995117188e-05\\
21	1.60446166992188e-05\\
22	1.45034790039063e-05\\
};

%+++++++ MCMA +++++++++
\addplot %MCMA
  table[row sep=crcr]{%
12	0.272158436414402\\
13	0.188032101230479\\
14	0.119150368494529\\
15	0.0686895230674329\\
16	0.0358239018213694\\
17	0.0168980633745658\\
18	0.00727839193532677\\
19	0.00293043245349177\\
20	0.00114109119833772\\
21	0.000452469075679362\\
22	0.000190326612772313\\
};

%+++++++ Louchet +++++++++
\addplot %Louchet
  table[row sep=crcr]{%
12	0.234100378234473\\
13	0.15308102009675\\
14	0.0898410684718029\\
15	0.0464115856628032\\
16	0.0205804357001396\\
17	0.00763803934937177\\
18	0.00230447063407032\\
19	0.000548926982890166\\
20	0.000139605856952697\\
21	0.000164353430083439\\
22	4.15083925846563e-05\\
};

%+++++++ UDDLMS +++++++++
% \addplot %
%   table[row sep=crcr]{%
% 12	0.230185294308626\\
% 13	0.148997832862569\\
% 14	0.0862149280867504\\
% 15	0.0436257345540729\\
% 16	0.0188057205934872\\
% 17	0.00671083731047693\\
% 18	0.00189876140385052\\
% 19	0.000409662023960261\\
% 20	6.17187753644362e-05\\
% 21	6.34719651959352e-06\\
% 22	3.7336450115256e-07\\
% };

%+++++++ Czegledi +++++++++
\addplot %Czegledi
  table[row sep=crcr]{%
12	0.229022523619363\\
13	0.147398079607805\\
14	0.0845530421090224\\
15	0.0422491315217038\\
16	0.0178888510113308\\
17	0.00622526866010844\\
18	0.00171039901301906\\
19	0.00034868186097854\\
20	5.0891204831012e-05\\
21	4.80503879744164e-06\\
22	2.92198305249829e-07\\
};

%+++++++SW-Kabsch+++++++++

\addplot %SW-Kabsch
  table[row sep=crcr]{%
12	0.227776208564657\\
13	0.144794990422389\\
14	0.0819214473556053\\
15	0.0402807132885296\\
16	0.0167021606441349\\
17	0.0056336807246518\\
18	0.00147836920879192\\
19	0.000281938898087725\\
20	3.66871205480341e-05\\
21	2.85705009577611e-06\\
22	1.46099152624915e-07\\
};
\end{axis}
%*************

%=================================================================
%                   Figure 3 DeltaP_T 3.57e-5
%=================================================================
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(2*\w cm+2cm,0cm)},
scale only axis,
font=\small,
xmin = \xMin=12,
xmax = \xMax,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax=1,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
xticklabels={$\text{12}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
%ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black}
]
\pgfplotsset{cycle list name=list1}
%+++++++++++ AWGN+++++++++++ 
\addplot %[color=ML_Demod, line width=1.0pt, mark=*]
  table[row sep=crcr]{%
12	0.203999794006348\\
13	0.129312927246094\\
14	0.0725995941162109\\
15	0.0351876449584961\\
16	0.0142747344970703\\
17	0.00464553070068359\\
18	0.0011612548828125\\
19	0.000215400695800781\\
20	3.66744995117188e-05\\
21	1.60446166992188e-05\\
22	1.45034790039063e-05\\
};

%+++++++++++ MCMA+++++++++++ 
\addplot %[color=Mcma, line width=1.0pt]
  table[row sep=crcr]{%
12	0.391968840297393\\
13	0.306107991623649\\
14	0.230668143891432\\
15	0.168168249407487\\
16	0.119854371611311\\
17	0.0848340070127593\\
18	0.0606591669101652\\
19	0.0444508376351417\\
20	0.033715293334632\\
21	0.0265755007954287\\
22	0.0217393104119996\\
};

%+++++++++++ UDDLMS+++++++++++ 
% \addplot %[color=LS, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.429521776890361\\
% 13	0.270835987467939\\
% 14	0.146883972922957\\
% 15	0.0697918817570858\\
% 16	0.0298411171715204\\
% 17	0.0112029804227135\\
% 18	0.0036831596376741\\
% 19	0.00100522710301614\\
% 20	0.000228361092172333\\
% 21	4.23362877828642e-05\\
% 22	7.05334242394727e-06\\
% };

%+++++++++++ Louchet+++++++++++ 
\addplot %[color=LS_DDLMS, line width=1.0pt]
  table[row sep=crcr]{%
12	0.364393980714912\\
13	0.262124176163112\\
14	0.176297677023473\\
15	0.113027669556183\\
16	0.0688472452193111\\
17	0.0413365475146911\\
18	0.0248860832440505\\
19	0.0154395474172916\\
20	0.0102473377487744\\
21	0.00678153306710821\\
22	0.00489939450017856\\
};

%+++++++++++ Czegledi+++++++++++ 
\addplot %[color=LS_Czegledi, line width=1.0pt]
  table[row sep=crcr]{%
12	0.294615044966072\\
13	0.192365410213954\\
14	0.11564026330314\\
15	0.0628165887471186\\
16	0.0305152430115905\\
17	0.0131026508879582\\
18	0.00498658322781728\\
19	0.00170010713937859\\
20	0.000528846466023831\\
21	0.000158184799194832\\
22	4.65406967306256e-05\\
};

%+++++++++++ SW-Kabsch+++++++++++ 
\addplot %[color=LS_SW_Kabsch, line width=1.0pt]
  table[row sep=crcr]{%
12	0.255571921366189\\
13	0.16429575338463\\
14	0.0948819681179182\\
15	0.0491095905977079\\
16	0.0225148452972306\\
17	0.00895018018895491\\
18	0.0030423038213045\\
19	0.000888972760624655\\
20	0.000221510665238142\\
21	4.86591344436869e-05\\
22	9.88604266095256e-06\\
};
\end{axis}
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax = \yMax,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}

\node at (0.5*\w,1*\h){{(a)}};
\node at (\w+1+0.5*\w,1*\h){{(b)}};
\node at (2*\w+2+0.5*\w,1*\h){{(c)}};


% \node at (0.5*\w,.85*\h)[font=\small]{$\Delta_p\cdot T = 10^{-8}$};
% \draw [black,very thick](0.18*\w,0.92*\h) rectangle (0.82*\w,.78*\h);

% \node at (\w+1+0.5*\w,.85*\h)[font=\small]{$\Delta_p\cdot T = 3.57\cdot 10^{-6}$};
% \draw [black,very thick](\w+1+0.18*\w,0.92*\h) rectangle  (\w+1+0.82*\w,.78*\h);

% \node at (2*\w+2+0.5*\w,.85*\h)[font=\small]{$\Delta_p\cdot T = 3.57\cdot 10^{-5}$};
% \draw [black,very thick](2*\w+2+0.18*\w,0.92*\h) rectangle (2*\w+2+0.82*\w,.78*\h);
\end{tikzpicture}%

==> Figures/tikz/Fig7.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{ML}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{LS}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{LS-DDLMS}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{LS-Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{LS-SW-Kabsch}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{SW-LS}{rgb}{0.92900,0,0.92}%

\newcommand\w{5}
\newcommand\h{4.5}
\newcommand\LineWidth{1.2}

\newcommand\xMax{20}
\newcommand\xMin{12}
\newcommand\yMax{1}

\pgfplotscreateplotcyclelist{list1}{%
{color=ML,mark=triangle*,line width=\LineWidth pt},
{color=MCMA,mark=+,line width=\LineWidth pt},
{color=LS,mark=x,line width=\LineWidth pt},
{color=LS-DDLMS,mark=star,line width=\LineWidth pt},
{color=LS-Czegledi,mark=o,line width=\LineWidth pt},
{color=LS-SW-Kabsch,mark=square,line width=\LineWidth pt},
{color=SW-LS,mark=diamond,line width=\LineWidth pt},
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0*\w cm,0*\w cm)},
scale only axis,
font=\small,
xmin=\xMin,
xmax=\xMax,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
%tick label style={font =\thin},
xticklabels={$\text{8}$,$\text{10}$,$\text{12}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black},
legend style={at={(0.25,1.1)},font=\footnotesize, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
legend columns=7
]

\pgfplotsset{cycle list name=list1}
\addplot %ML
  table[row sep=crcr]{%
12	0.121984935\\
13	0.076938405\\
14	0.043715635\\
15	0.02197132\\
16	0.00958871\\
17	0.003566395\\
18	0.00110248\\
19	0.000273825\\
20	5.28849999999999e-05\\
21	7.71e-06\\
22	8.2e-07\\
};
\addlegendentry{ML ($\Hb$ is known)}

\addplot
  table[row sep=crcr]{%
12	0.274425559456877\\
13	0.19083771306029\\
14	0.121325040556457\\
15	0.0700027000600013\\
16	0.036195154336763\\
17	0.0161629980666237\\
18	0.00626647258827974\\
19	0.002221649369986\\
20	0.000625447232160714\\
21	0.000224321651592257\\
22	2.59172426053912e-05\\
};
\addlegendentry{MCMA}

\addplot
  table[row sep=crcr]{%
12	0.15577995\\
13	0.10576081\\
14	0.066120385\\
15	0.037403595\\
16	0.01881511\\
17	0.008239335\\
18	0.003074405\\
19	0.000948505\\
20	0.000235385\\
21	4.65399999999999e-05\\
22	6.95e-06\\
};
\addlegendentry{LS}

\addplot 
  table[row sep=crcr]{%
12	0.14455214\\
13	0.094584635\\
14	0.056582635\\
15	0.03040727\\
16	0.01441712\\
17	0.005893495\\
18	0.00202646\\
19	0.000569275\\
20	0.000126995\\
21	2.2e-05\\
22	2.87e-06\\
};
\addlegendentry{LS-DDLMS}

% \addplot 
%   table[row sep=crcr]{%
% 12	0.21118235\\
% 13	0.15294896\\
% 14	0.10354584\\
% 15	0.064715285\\
% 16	0.03676051\\
% 17	0.018808255\\
% 18	0.00843478\\
% 19	0.00330759\\
% 20	0.0011273\\
% 21	0.00033962\\
% 22	8.5235e-05\\
% };
% \addlegendentry{LS-UDDLMS}

\addplot 
  table[row sep=crcr]{%
12	0.147787105\\
13	0.09889277\\
14	0.06071321\\
15	0.033525655\\
16	0.01636136\\
17	0.00688642\\
18	0.002440735\\
19	0.00070594\\
20	0.000160985\\
21	2.892e-05\\
22	3.89e-06\\
};
\addlegendentry{LS-Czegledi}

\addplot 
  table[row sep=crcr]{%
12	0.16247272\\
13	0.107852825\\
14	0.06586971\\
15	0.036307395\\
16	0.01771763\\
17	0.00747701\\
18	0.00266229\\
19	0.000776005\\
20	0.00017812\\
21	3.2105e-05\\
22	4.335e-06\\
};
\addlegendentry{LS-SW-Kabsch}

\addplot 
  table[row sep=crcr]{%
12	0.164937535\\
13	0.10702361\\
14	0.0637649\\
15	0.03427869\\
16	0.016335075\\
17	0.00674878\\
18	0.00236041\\
19	0.00067716\\
20	0.00015414\\
21	2.8255e-05\\
22	3.64e-06\\
};
\addlegendentry{SW-LS}


\end{axis}

%=================================================================
%                   Figure 2 Deltap_T = 3.57 e-6
%=================================================================
%-************
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(\w cm+1cm,0 cm)},
scale only axis,
xmin=\xMin,
xmax=\xMax,
font=\small,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
%tick label style={font =\thin},
xticklabels={$\text{8}$,$\text{10}$,$\text{12}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
%ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black}
]

\pgfplotsset{cycle list name=list1}
\addplot
  table[row sep=crcr]{%
12	0.12187766\\
13	0.07689393\\
14	0.043693015\\
15	0.021996085\\
16	0.00961379\\
17	0.00357489\\
18	0.00109853\\
19	0.00027401\\
20	5.2695e-05\\
21	7.59500000000001e-06\\
22	8.55e-07\\
};
%\addlegendentry{ML}
\addplot
  table[row sep=crcr]{%
12	0.304594374319429\\
13	0.220439676437254\\
14	0.148438070846019\\
15	0.092409809106869\\
16	0.0530058667970399\\
17	0.0278799306651259\\
18	0.013610091335363\\
19	0.00620251561145803\\
20	0.00271072690504234\\
21	0.00117871508255739\\
22	0.000538367519278206\\
};
%\addlegendentry{MCMA}

\addplot
  table[row sep=crcr]{%
12	0.260048915\\
13	0.218387525\\
14	0.182857175\\
15	0.15376105\\
16	0.13067765\\
17	0.11293832\\
18	0.099634095\\
19	0.08964495\\
20	0.08222633\\
21	0.076597715\\
22	0.07239447\\
};
%\addlegendentry{LS}

\addplot 
  table[row sep=crcr]{%
12	0.174540235\\
13	0.11346517\\
14	0.06862287\\
15	0.0381236\\
16	0.019149915\\
17	0.008574335\\
18	0.003395635\\
19	0.00117789\\
20	0.000360425\\
21	9.901e-05\\
22	2.4795e-05\\
};
%\addlegendentry{LS-DDLMS}

% \addplot [color=myLS-DDLMS, line width=2.0pt]
%   table[row sep=crcr]{%
% 12	0.21118235\\
% 13	0.15294896\\
% 14	0.10354584\\
% 15	0.064715285\\
% 16	0.03676051\\
% 17	0.018808255\\
% 18	0.00843478\\
% 19	0.00330759\\
% 20	0.0011273\\
% 21	0.00033962\\
% 22	8.5235e-05\\
% };
% \addlegendentry{LS-UDDLMS}

\addplot 
  table[row sep=crcr]{%
12	0.1678503\\
13	0.11452835\\
14	0.072531205\\
15	0.042137645\\
16	0.02220963\\
17	0.010517145\\
18	0.004485255\\
19	0.0017495\\
20	0.000658805\\
21	0.00025843\\
22	0.000118645\\
};
%\addlegendentry{LS-Czegledi}

\addplot 
  table[row sep=crcr]{%
12	0.168700535\\
13	0.113717055\\
14	0.071169835\\
15	0.04086773\\
16	0.021238885\\
17	0.00988296\\
18	0.004119315\\
19	0.00156077\\
20	0.00057097\\
21	0.00021942\\
22	9.9475e-05\\
};
%\addlegendentry{SW-Kabsch}

\addplot
 table[row sep=crcr]{%
12	0.16812662\\
13	0.109171085\\
14	0.065148175\\
15	0.0352107\\
16	0.016934555\\
17	0.007094695\\
18	0.002529155\\
19	0.000748705\\
20	0.000182055\\
21	3.4585e-05\\
22	5.29500000000001e-06\\
};
%\addlegendentry{SW-LS}

\end{axis}
%*************

%=================================================================
%                   Figure 3 DeltaP_T 3.57e-5
%=================================================================
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(2*\w cm+2cm,0 cm)},
scale only axis,
xmin=\xMin,
xmax=\xMax,
font=\small,
xlabel style={font=\small\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
%tick label style={font =\thin},
xticklabels={$\text{8}$,$\text{10}$,$\text{12}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\small\color{white!15!black}},
% ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black}
]
\pgfplotsset{cycle list name=list1}
\addplot 
  table[row sep=crcr]{%
12	0.121956985\\
13	0.07694169\\
14	0.043788665\\
15	0.022032315\\
16	0.00963232500000001\\
17	0.003598475\\
18	0.00111444\\
19	0.000277925\\
20	5.4635e-05\\
21	8.26e-06\\
22	7.85e-07\\
};

\addplot
  table[row sep=crcr]{%
12	0.468244399875553\\
13	0.362538917531501\\
14	0.275811406920154\\
15	0.204127625058335\\
16	0.15076867263717\\
17	0.109440654236761\\
18	0.0801263139180871\\
19	0.0597025989466433\\
20	0.0457735060779128\\
21	0.0362821062690282\\
22	0.02974373874975\\
};
%\addlegendentry{MCMA}

\addplot 
  table[row sep=crcr]{%
12	0.58228452\\
13	0.56760386\\
14	0.554938195\\
15	0.54424801\\
16	0.535544665\\
17	0.52853399\\
18	0.522750595\\
19	0.51818047\\
20	0.51467562\\
21	0.511783485\\
22	0.509513035\\
};
%\addlegendentry{LS}

\addplot 
  table[row sep=crcr]{%
12	0.49487822\\
13	0.38046892\\
14	0.26751925\\
15	0.173192685\\
16	0.10593021\\
17	0.06243529\\
18	0.036590305\\
19	0.02201537\\
20	0.013735735\\
21	0.009118145\\
22	0.006475225\\
};
%\addlegendentry{LS-DDLMS}

% \addplot 
%   table[row sep=crcr]{%
% 12	0.383175605\\
% 13	0.30051266\\
% 14	0.222237375\\
% 15	0.15600744\\
% 16	0.107198065\\
% 17	0.07297335\\
% 18	0.050597845\\
% 19	0.036392625\\
% 20	0.0274308\\
% 21	0.02196765\\
% 22	0.018383675\\
% };
% %\addlegendentry{LS-UDDLMS}

\addplot 
  table[row sep=crcr]{%
12	0.2532437\\
13	0.191785455\\
14	0.141466535\\
15	0.1031662\\
16	0.07556732\\
17	0.05636168\\
18	0.043667215\\
19	0.035364445\\
20	0.029913525\\
21	0.02636263\\
22	0.023837545\\
};
%\addlegendentry{LS-Czegledi}


\addplot 
  table[row sep=crcr]{%
12	0.229692425\\
13	0.17103033\\
14	0.12427022\\
15	0.08938962\\
16	0.06494567\\
17	0.04830244\\
18	0.03736626\\
19	0.0304646\\
20	0.02596965\\
21	0.023124265\\
22	0.02113808\\
};
%\addlegendentry{SW-Kabsch}

\addplot 
  table[row sep=crcr]{%
12	0.21963346\\
13	0.145360605\\
14	0.088718675\\
15	0.049865925\\
16	0.025634655\\
17	0.01201504\\
18	0.005116875\\
19	0.00201328\\
20	0.00076296\\
21	0.00028471\\
22	0.000122995\\
};
%\addlegendentry{SW-LS}

\end{axis}
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax = \yMax,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}

\node at (0.5*\w,1*\h){{(a)}};
\node at (\w+1+0.5*\w,1*\h){{(b)}};
\node at (2*\w+2+0.5*\w,1*\h){{(c)}};


% \node at (0.3*\w,.1*\h)[font=\small]{$\Delta_p\cdot T = 10^{-8}$};
% \draw [black,very thick](0.03*\w,0.17*\h) rectangle (0.6*\w,.04*\h);

% \node at (\w+1+0.32*\w,.1*\h)[font=\small]{$\Delta_p\cdot T = 3.57\cdot 10^{-6}$};
% \draw [black,very thick](\w+1+0.03*\w,0.17*\h) rectangle  (\w+1+0.62*\w,.04*\h);

% \node at (2*\w+2+0.32*\w,.1*\h)[font=\small]{$\Delta_p\cdot T = 3.57\cdot 10^{-5}$};
% \draw [black,very thick](2*\w+2+0.03*\w,0.17*\h) rectangle (2*\w+2+0.62*\w,.04*\h);
\end{tikzpicture}%
